Bounding the Distance to Unsafe Sets with Convex Optimization

This work proposes an algorithm to bound the minimum distance between points on trajectories of a dynamical system and points on an unsafe set. Prior work on certifying safety of trajectories includes barrier and density methods, which do not provide a margin of proximity to the unsafe set in terms of distance. The distance estimation problem is relaxed to a Monge-Kantorovich type optimal transport problem based on existing occupation-measure methods of peak estimation. Specialized programs may be developed for polyhedral norm distances (e.g. L1 and Linfinity) and for scenarios where a shape is traveling along trajectories (e.g. rigid body motion). The distance estimation problem will be correlatively sparse when the distance objective is separable.

==> section/biography.tex <==
\vspace{-0.5cm}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{img/jared_kdd_small (1).jpg}}]{Jared Miller}  is currently a Research Assistant (\rw{5}th-year Ph.D. student) at the Robust Systems Laboratory in Northeastern University. He received his B.S. and M.S. degrees in Electrical Engineering from Northeastern University in 2018. He is a recipient of the 2020 Chateaubriand Fellowship from the Office for Science Technology of the Embassy of France in the United States. He was given an Outstanding Student Paper award at the \rw{IEEE} Conference on Decision and Control in 2021 \rw{and in 2022}. His research interests include large-scale convex optimization, semi-algebraic geometry, measure theory, and analysis of nonlinear systems.
\end{IEEEbiography}

\vspace{-0.5cm}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{img/Mario18.png}}]{Mario Sznaier}  is currently the Dennis Picard Chaired Professor at the
Electrical and Computer Engineering Department, Northeastern University,
Boston. Prior to joining Northeastern University, Dr. Sznaier
was a Professor of Electrical Engineering at the Pennsylvania State
University and also held visiting positions at the California Institute
of Technology. 
His research interest include robust identification and
control of hybrid systems, robust optimization, and dynamical vision.
Dr. Sznaier is currently serving as Editor in Chief of the section on AI and Control of the journal Frontiers in Control Engineering, and chair of IFAC’s Technical Committee TC 2.5.
Additional  service
includes  Associate Editor for the Journal Automatica (2005-2021),  chair of the CSS Technical Committee on Computational
Aspects of Control System Design (2012-2016), General co-Chair of the 2016 MSC, and Program Chair of the 2017 CDC.
He is a
distinguished member of the IEEE Control Systems Society and an IEEE Fellow.
\end{IEEEbiography}
